Random pinning in glassy spin models with plaquette interactions

We use a random pinning procedure to study amorphous order in two glassy spin models. On increasing the concentration of pinned spins at constant temperature, we find a sharp crossover (but no thermodynamic phase transition) from bulk relaxation to localisation in a single state. At low temperatures, both models exhibit scaling behaviour. We discuss the growing length and time scales associated with amorphous order, and the fraction of pinned spins required to localize the system in a single state. These results, obtained for finite dimensional interacting models, provide a theoretical scenario for the effect of random pinning that differs qualitatively from previous approaches based either on mean-field, mode-coupling, or renormalization group reatments.

==> PaxHeader/pmpin_cm.tex <==
18 gid=1552001941
18 uid=1632763755
20 ctime=1323256634
20 atime=1323256662
38 LIBARCHIVE.creationtime=1323255234
24 SCHILY.dev=234881026
23 SCHILY.ino=12200861
18 SCHILY.nlink=1

